The SWAP Filter: A Simple Azimuthally Varying Radial Filter for Wide-Field EUV Solar Images

We present the SWAP Filter: an azimuthally varying, radial normalizing filter specifically developed for EUV images of the solar corona, named for the Sun Watcher with Active Pixels and Image Processing (SWAP) instrument on the Project for On-Board Autonomy 2 spacecraft. We discuss the origins of our technique, its implementation and key user-configurable parameters, and highlight its effects on data via a series of examples. We discuss the filter's strengths in a data environment in which wide field-of-view observations that specifically target the low signal-to-noise middle corona are newly available and expected to grow in the coming years.

==> oldstuff.tex <==
\section{Controlling Dynamic Range}

One of the key problems in the display of coronal image data is determining effective approaches to displaying image data where the dynamic range spans many orders of magnitude, something that is a particular problem in observations in the extreme-ultraviolet (EUV). Here, the corona is highly structured and highly dynamic. Bright structures in solar flares can produce several 1000~$\mathrm{W}/\mathrm{m}^2\,\mathrm{sr}^{-1}$ while faint structures in the outer corona might produce only $10^{-6}$ that radiance. So it is probably not surprising that finding methods to visualize images such that the six or seven orders of magnitude of dynamic range possible in the corona is displayed adequately, and coherent structures are preserved, is a question that has spawned substantial research.

Gamma adjustment (scaling)???

Although the present-day problem is generally tackled via digital image processing techniques, the most famous approach to it predates electronic imaging systems by decades. Gordon Newkirk, frustrated that photographic images could not handle sufficient dynamic range to capture the detail in the corona visible by eye during a total solar eclipse, devised a radially graded neutral-density filter that successfully compensated for the steep brightness gradient of the corona \citep{Eddy1989}. Newkirk first deployed his filter at an eclipse in 1966 in Bolivia, generating a stunning image of the corona that arguably actually revealed more detail than was visible to eye \citep{1967ARA&A...5..213N}. Subsequently, Newkirk-style filters were widely used for eclipse photography before digital imaging made it possible to assemble high-dynamic range (HDR) composites using multiple exposure times instead of radial normalizing filters.

Still, even if we can now routinely make high-quality, HDR images of the corona there is a need for processing tools can make them displayable on screens that have extremely limited dynamic range. \citet{1988sscd.conf..256K} achieved maybe the earliest success in this sort of digital filtering with an algorithm they referred to as ``Mad MAXII,'' which used two-dimensional second derivatives to amplify high-frequency, coherent features in solar images. \citet{2000ASPC..205..101E} also obtained good results using filtering techniques available in \textsf{Adobe Photoshop}. 

More recently, a series of authors have advanced a class of related techniques they refer to as normalizing-radial-graded filters. \citet{2006CoSka..36..131D} discussed the composition of HDR eclipse images via multiple exposures and a radial blur procedure that attempts to draw upon the strengths in human vision that allow us to detect fine details even in images with a wide dynmic range. This basic approach was further developed in papers by \citep{2006SoPh..236..263M, 2011ApJ...737...88D}, which filter the image by decomposing the image into a series of small, circular subregions, the properties of which allow the removal of the steep brightness gradient and adjustment of image contrast as a function of height in a coronal image. These are powerful techniques, and they have become standard in the processing of eclipse images to enhance the fine structure of the corona.

Other approaches, which have been deployed successfully on EUV images in particular, use multiscale processing techniques based on both wavelet techniques \citep{2008ApJ...674.1201S} and Gaussian normalizaton approaches \citep{2013ApJS..207...25D, 2014SoPh..289.2945M}. These processing techniques, too, are powerful, dramatically improving the visibility of fine, faint structures in EUV coronal images. One limitation, however, is that they are computationally expensive, and can take as long as several minutes to run on a single image. Another limitation is that the resulting images often do not look ``natural,'' and thus the results can be sometimes difficult to interpret, since the connection between the corona's inherent properties and the resulting image is largely lost.

Some of us first started thinking about this problem when we began exploring the evolution of the corona on very large scales with SWAP \citep{2013ApJ...777...72S}. In trying to generate images that showed the wide range of coronal brightness on the largest scales, but still had an overall natural appearance, we realized that EUV image filters must successfully balance several competing priorities. They must sufficiently reduce the dynamic range of an image that it can be displayed relatively uniformly without suppressing the contrast more locally such that the fine features in the image become invisible. They must enhance high-frequency structure such that fine, coherent features are visible across their full extent, but ideally should avoid oversharpening the image such that processing produces artifacts. Nor should they over-enhance noise in the image.

Since this approach was intended to be run on movies that were thousands of images long and spanned multiple Carrington rotations, an additional goal was to develop an approach that could work quickly and thus minimize the processing time to generating a filtered movie. Ideally, a single filter would achieve uniformly good results on a variety of images as the sun changed throughout the duration of the movie. 

The most straightforward approach to this problem is to devise a uniform radial normalizing filter---one that acts essentially as a digital version of Newkirk's optical filter---to normalize the falloff in coronal brightness as a function of height at all azimuths. But this approach suffers from a number of key limitations. First, the coronal falloff is not the same at all azimuths \citep[see, for example][]{1997ASIC..494..159K} so a filter that performs well at the equator might not perform very well at the poles and vice versa. Second, this method provides a means to normalize the coronall falloff above the limb, but what is the best way to treat the disk using this approach? This approach provides no clear path towards a single image filter that will perform well on a variety of conditions and handle the wide variation in the appearance of the corona at a variety of azimuths.

FIGURE?

A second possibility is to normalize the image with a highly smoothed version of itself. Such an approach has the advantage that the normalization filter will adapt to changing conditions as a function of azimuth, but this, too, has important limitations. Foremost is that the smoothing widens the brightness at the solar limb in the filter too much, meaning that structures near the limb can become ``over-normalized,'' reducing the resulting filtered image's intrinsic brightness too much in the region near the limb, leading to image artifacts. In practice, it turns out that an approach like this one largely acts as a crude high-pass filter; it is difficult to obtain a result that resembles a natural solar image. The approach might have some merit for certain applications, but it doesn't achieve the original goal.

FIGURE?

Such failed attempts at filters help define the qualities a successful filter must have. Azimuthally, it must be capable of adapting to the prevailing conditions: relatively weak and fast-decaying signals near the polar coronal holes and brighter, more extended signal near the equatorial streamer belt. It also must decline radially rapidly enough that it does not introduce artifacts at the limb or elsewhere, but must not be so sensitive to the changing dynamic range of the corona that it acts as a high-pass filter. One way to produce a filter with these properties, it turned out, was to take the median value in each pixel over the long-duration image stack. This approach yields a smooth filter that will be dark anywhere the corona is mainly dark for at least half of the time period of interest, and likewise for regions that are predominantly bright.

FIGURE


